Boosting Weakly Supervised Object Detection using Fusion and Priors from Hallucinated Depth

Despite recent attention and exploration of depth for various tasks, it is still an unexplored modality for weakly-supervised object detection (WSOD). We propose an amplifier method for enhancing the performance of WSOD by integrating depth information. Our approach can be applied to any WSOD method based on multiple-instance learning, without necessitating additional annotations or inducing large computational expenses. Our proposed method employs a monocular depth estimation technique to obtain hallucinated depth information, which is then incorporated into a Siamese WSOD network using contrastive loss and fusion. By analyzing the relationship between language context and depth, we calculate depth priors to identify the bounding box proposals that may contain an object of interest. These depth priors are then utilized to update the list of pseudo ground-truth boxes, or adjust the confidence of per-box predictions. Our proposed method is evaluated on six datasets (COCO, PASCAL VOC, Conceptual Captions, Clipart1k, Watercolor2k, and Comic2k) by implementing it on top of two state-of-the-art WSOD methods, and we demonstrate a substantial enhancement in performance.

==> background.tex <==
\section{Background}

The following section will provide an overview of MIL-based WSOD, which will serve as the background for introducing our proposed method in the subsequent sections.

Specifically, let denote $\mathbf{I} \in \mathbb{R}^{h\times w \times 3}$ as an RGB image, $y_c \in \{0, 1\}$ where $c \in \{1, . . . , C\}$ as its corresponding ground-truth class labels
%, and $\mathbf{R} \in \mathbb{R}^{4\times N }$ as the precomputed object proposals. 
where C is the total number of object categories. Let $v_i$ where $i \in \{1, . . . , R\}$ to denote the visual regions $\mathbf{v}$ of a given image $\mathbf{I}$ where R is the number of proposals. With the help of a pre-trained backbone model, the feature map $\psi(\mathbf{I})$ is extracted, and proposal feature vectors are extracted by an RoI pooling layer. Finally, a box feature extractor is applied to extract a fixed-length feature vector $\phi(v_i)$ for each visual region. The proposal features $\phi(v_i)$ are fed into two parallel fully-connected layers to compute the visual detection score $v^{det}_{i,c} \in \mathbb{R}^1$ and classification score $v^{cls}_{i,c} \in \mathbb{R}^1$: %which are dependent to particular class c and visual region $v_i$:

\begin{equation}
   v^{det}_{i,c} = w^{det\intercal}_{c} \phi(v_i) + b^{det}_{c}, \quad v^{cls}_{i,c} = w^{cls\intercal}_{c} \phi(v_i) + b^{cls}_{c}
   \label{eq:1}
\end{equation}

 where $w$ and $b$ are weight and bias parameters, respectively.


 
 %These classification and detection scores are converted to probabilities such that $vp^{cls}_{i,c}$ is the probability that class $c$ is in present proposal $v_i$, and $vp^{det}_{i,c}$ is the probability that $v_i$ is important for predicting image-level label $y_c$.

%\begin{equation}
%   vp^{det}_{i,c} = \dfrac{exp(v^{det}_{i,c})} {\sum_{k=1}^{N} exp(v^{det}_{k,c})}, \quad vp^{cls}_{i,c} = \dfrac{exp(v^{cls}_{i,c})} {\sum_{k=1}^{C} exp(v^{cls}_{i,k})}
%   \label{eq:2}
%\end{equation}

%Element-wise multiplication of classification and detection score probabilities results in $vp^{comb}_{i,c}$. Finally, visual aggregated image-level predictions $\hat{vp}_c$ are computed as follows, where greater values of $\hat{vp}_c\in [0, 1]$  mean higher likelihood that $c$ is present in the image.

%\begin{equation}
%  vp^{comb}_{i,c} = vp^{det}_{i,c} vp^{cls}_{i,c}, \quad  \hat{vp}_c = \sigma\left(\sum_{i=1}^{M}vp^{comb}_{i,c} \right)
%  \label{eq:confidence}
%\end{equation}

%Assuming the label $y_c$ = 1 if and only if class $c$ is present, the visual classification loss used for training the model is defined as follows. Again, since no region-level labels are provided, region-level scores are derived indirectly, by optimizing this loss.

%\begin{equation}
%    \mathcal{L}_{mil} = -\sum_{c=1}^{C}\left[ y_c\log\hat{vp}_c + (1-y_c)\log(1-\hat{vp}_c) \right]
%    \label{eq:visual_loss}
%\end{equation}

==> table_anno_percent.tex <==
%\begin{table*}[t]
%\centering
%\resizebox{2.05\columnwidth}{!}{
%\begin{tabular}{ lcc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
%\toprule
 %& \multicolumn{3}{c}{Avg. Precision, IoU}  & \multicolumn{3}{c}{Avg. Precision, Area} \\
 %\cmidrule{2-4} \cmidrule{5-7}

 %& \multicolumn{3}{c}{Avg. Precision, IoU}\\
 %\cmidrule{2-4}
%\% of GT anno. & \multicolumn{2}{c}{person}&\multicolumn{2}{c}{car}&\multicolumn{2}{c}{motorcycle}&\multicolumn{2}{c}{handbag}&\multicolumn{2}{c}{bowl}&\multicolumn{2}{c}{hair drier}&\multicolumn{2}{c}{toaster}&\multicolumn{2}{c}{scissors}&\multicolumn{2}{c}{parking meter}&\multicolumn{2}{c}{tennis racket}  \\

%\midrule 

%\textsc{1\%}  &0.23&0.49&0.26&0.53&0.17&0.43&0.13&0.41&0.13&0.43&0.39&0.52&0.32&0.42&0.08&0.42&0.11&0.39&0.23&0.48\\

%\textsc{5\%} 
%&0.23&0.49&0.28&0.54&0.15&0.41&0.14&0.41&0.13&0.43&0.22&0.46&0.27&0.55&0.15&0.45&0.12&0.35&0.16&0.44\\

%\textsc{10\%}
%&0.23&0.49&0.28&0.54&0.16&0.41&0.14&0.42&0.13&0.43&0.27&0.47&0.26&0.54&0.15&0.46&0.16&0.44&0.16&0.43\\

%\textsc{50\%}
%&0.23&0.49&0.27&0.54&0.16&0.42&0.15&0.42&0.14&0.44&0.24&0.50&0.26&0.54&0.16&0.45&0.15&0.44&0.17&0.44\\
%\midrule 
%\textsc{Average}
%&0.230&0.490&0.272&0.537&0.160&0.417&0.140&0.415&0.132&0.432&0.280&0.487&0.277&0.512&0.135&0.445&0.135&0.405&0.180&0.447\\
%\textsc{Stdev}
%&0&0&0.009&0.005&0.008&0.009&0.008&0.005&0.005&0.005&0.070&0.027&0.028&0.061&0.036&0.017&0.023&0.043&0.033&0.022\\

%\bottomrule
%\hline \\
%\end{tabular}}
%\caption{The table displays the lower and upper depth range values, denoted as $r_c = [\text{lower}, \text{upper}]$, for each object class $c$, which are extracted using varying percentages of ground truth bounding box annotations.
%, such as $1\%$, $5\%$, $10\%$, and $50\%$. 
%Among the ten object classes considered, the first 5 %, namely person, car, motorcycle, handbag, and bowl, 
%exhibit the lowest standard deviations across the different percentages, and the last 5 %, including hair drier, toaster, scissors, parking meters, and tennis racket, 
%display the highest deviations out of the 80 COCO classes.} % for visual methods.} 
%\label{Table:4}
%\end{table*}

\begin{table*}[t]
\centering
\resizebox{2.05\columnwidth}{!}{
\begin{tabular}{ cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
 \multicolumn{2}{c}{person}&\multicolumn{2}{c}{car}&\multicolumn{2}{c}{motorcycle}&\multicolumn{2}{c}{handbag}&\multicolumn{2}{c}{bowl}&\multicolumn{2}{c}{hair drier}&\multicolumn{2}{c}{toaster}&\multicolumn{2}{c}{scissors}&\multicolumn{2}{c}{parking meter}&\multicolumn{2}{c}{tennis racket}  \\

\midrule 
0.23&0.49&0.26&0.53&0.17&0.43&0.13&0.41&0.13&0.43&0.39&0.52&0.32&0.42&0.08&0.42&0.11&0.39&0.23&0.48\\


\bottomrule
\hline \\
\end{tabular}}
\caption{The table displays the lower and upper depth range values per object, denoted as $r_c = [\text{lower}, \text{upper}]$. While the first 5 objects have a smaller depth value, the last 5 objects have larger depth values.} % for visual methods.} 
\label{Table:4}
\end{table*}


